Distilling Symbolic Priors for Concept Learning into Neural Networks

Humans can learn new concepts from a small number of examples by drawing on their inductive biases. These inductive biases have previously been captured by using Bayesian models defined over symbolic hypothesis spaces. Is it possible to create a neural network that displays the same inductive biases? We show that inductive biases that enable rapid concept learning can be instantiated in artificial neural networks by distilling a prior distribution from a symbolic Bayesian model via meta-learning, an approach for extracting the common structure from a set of tasks. By generating the set of tasks used in meta-learning from the prior distribution of a Bayesian model, we are able to transfer that prior into a neural network. We use this approach to create a neural network with an inductive bias towards concepts expressed as short logical formulas. Analyzing results from previous behavioral experiments in which people learned logical concepts from a few examples, we find that our meta-trained models are highly aligned with human performance.

==> deleted.tex <==




Can we use the symbolic representations from Bayesian models to enable neural networks to acquire concepts from smaller amounts of data? Answering this question is important if we wish for neural networks to realize their potential as models of human learning and if we wish to translate Bayesian proposals into more plausible implementations.
This problem is at its core about \textit{inductive biases}---the factors that guide how a learner generalizes. Bayesian models are effective at capturing human inductive biases \cite<e.g.,>{goodman,piantadosi}. Therefore, if neural networks could be given the same inductive biases as Bayesian models, then they could match human learning behavior as effectively as Bayesian models do. 
%that matched those of humans, then they would automatically match human learning behavior. 
How, then, can a Bayesian model's inductive biases be given to a neural network?
we characterize human inductive biases, and how can we give those biases to neural networks?

%that matched those of humans, then they would automatically match human learning behavior. 

we characterize human inductive biases, and how can we give those biases to neural networks?

%, as demonstrated by their success in artificial intelligence (AI)---e.g., the popular ImageNet challenge \cite{imagenet} involves determining what class an image belongs to, where each class---e.g., \textit{canoe} or \textit{quail}---can be thought of as corresponding to a concept. The best-performing systems on ImageNet are neural networks (e.g., \citeNP{yu2022coca,chen2023pali}).
%When combined with the many desirable properties that originally motivated connectionism, such as the connections to neuroscience and the potential for modeling how higher cognition might emerge from simple algorithmic components \cite{mcclelland1986appeal}, this success in AI makes neural networks attractive as potential cognitive models.




